Learning on Large-scale Text-attributed Graphs via Variational Inference

This paper studies learning on text-attributed graphs (TAGs), where each node is associated with a text description. An ideal solution for such a problem would be integrating both the text and graph structure information with large language models and graph neural networks (GNNs). However, the problem becomes very challenging when graphs are large due to the high computational complexity brought by training large language models and GNNs together. In this paper, we propose an efficient and effective solution to learning on large text-attributed graphs by fusing graph structure and language learning with a variational Expectation-Maximization (EM) framework, called GLEM. Instead of simultaneously training large language models and GNNs on big graphs, GLEM proposes to alternatively update the two modules in the E-step and M-step. Such a procedure allows training the two modules separately while simultaneously allowing the two modules to interact and mutually enhance each other. Extensive experiments on multiple data sets demonstrate the efficiency and effectiveness of the proposed approach.

==> figures/att_ana_para.tex <==
\begin{figure}[t!]
    \small
    \centering
    {\setlength{\fboxsep}{0pt}\colorbox{white!0}{\parbox{0.85\textwidth}{\colorbox{red!14.970936}{\strut Who} \colorbox{red!13.802228}{\strut are} \colorbox{red!9.717735}{\strut the} \colorbox{red!6.521768}{\strut only} \colorbox{red!12.306012800000001}{\strut players} \colorbox{red!6.903509}{\strut listed} \colorbox{red!7.086827999999999}{\strut that} \colorbox{red!8.5836988}{\strut played} \colorbox{red!5.565175999999999}{\strut in} \colorbox{red!3.8364928}{\strut 2011} \colorbox{red!12.1032894}{\strut ?} \colorbox{red!9.142228999999999}{\strut [HEAD]} \colorbox{red!34.7230372}{\strut player} \colorbox{red!2.3756811}{\strut $|$} \colorbox{red!2.3478372000000003}{\strut year} \colorbox{red!2.7668154}{\strut $|$} \colorbox{red!5.4725796}{\strut round} \colorbox{red!2.8656236}{\strut $|$} \colorbox{red!3.826232}{\strut result} \colorbox{red!2.804299}{\strut $|$} \colorbox{red!5.366216799999999}{\strut opponent} \colorbox{red!2.9017952000000005}{\strut [ROW]} \colorbox{red!2.8313821999999997}{\strut 1} \colorbox{red!10.299296}{\strut ray} \colorbox{red!10.579882}{\strut mond} \colorbox{red!8.221680000000001}{\strut van} \colorbox{red!9.008807}{\strut bar} \colorbox{red!7.4133814}{\strut ne} \colorbox{red!6.2307126}{\strut ve} \colorbox{red!9.183715000000001}{\strut ld} \colorbox{red!3.4074528}{\strut $|$} \colorbox{red!3.1364577999999996}{\strut 2009} \colorbox{red!3.0261772}{\strut $|$} \colorbox{red!7.1568668}{\strut quarter} \colorbox{red!10.29556}{\strut -} \colorbox{red!7.359226}{\strut final} \colorbox{red!2.7560094}{\strut $|$} \colorbox{red!6.2080400000000004}{\strut won} \colorbox{red!3.2449352}{\strut $|$} \colorbox{red!8.8993174}{\strut j} \colorbox{red!10.114287200000001}{\strut elle} \colorbox{red!6.2276626}{\strut k} \colorbox{red!8.8740266}{\strut la} \colorbox{red!9.735318}{\strut as} \colorbox{red!7.475064000000001}{\strut en} \colorbox{red!3.1987599999999996}{\strut [ROW]} \colorbox{red!3.2400194}{\strut 2} \colorbox{red!9.723582799999999}{\strut ray} \colorbox{red!9.352703}{\strut mond} \colorbox{red!7.594534}{\strut van} \colorbox{red!8.3187848}{\strut bar} \colorbox{red!7.1613126}{\strut ne} \colorbox{red!6.573388}{\strut ve} \colorbox{red!9.092343999999999}{\strut ld} \colorbox{red!3.7991596000000003}{\strut $|$} \colorbox{red!3.5757356000000002}{\strut 2010} \colorbox{red!4.040925}{\strut $|$} \colorbox{red!8.162047999999999}{\strut 2} \colorbox{red!9.4804764}{\strut nd} \colorbox{red!8.9249826}{\strut round} \colorbox{red!3.7699683999999998}{\strut $|$} \colorbox{red!8.1906486}{\strut won} \colorbox{red!4.8999714}{\strut $|$} \colorbox{red!11.6535628}{\strut bre} \colorbox{red!13.612498}{\strut nd} \colorbox{red!12.360156}{\strut an} \colorbox{red!10.665865}{\strut d} \colorbox{red!12.203512000000002}{\strut olan} \colorbox{red!37.615702}{\strut [ROW]} \colorbox{red!42.653722}{\strut 3} \colorbox{red!55.65368000000001}{\strut ad} \colorbox{red!57.33528}{\strut rian} \colorbox{red!60.769768}{\strut le} \colorbox{red!61.41157200000001}{\strut w} \colorbox{red!61.32967}{\strut is} \colorbox{red!45.39855000000001}{\strut $|$} \colorbox{red!23.587676000000002}{\strut 2011} \colorbox{red!45.02534}{\strut $|$} \colorbox{red!40.120506}{\strut final} \colorbox{red!37.421062}{\strut $|$} \colorbox{red!33.088660000000004}{\strut won} \colorbox{red!38.722848}{\strut $|$} \colorbox{red!37.43384}{\strut g} \colorbox{red!38.099266}{\strut ary} \colorbox{red!21.687636}{\strut and} \colorbox{red!26.274652}{\strut erson} }}}
    \caption{\todo{this is a demo and should be replaced}}
\end{figure}

